Normality in the square of the Sorgenfrey Line

We consider sets of reals $X$ endowed with the Sorgenfrey lower limit topology denoted $X[\leq]$. Przymusi\'nski proved that if $X$ is a $Q$-set then $(X[\leq])^2$ is normal. While the converse is not in general true we consider examples of sets of the reals for which $(X[\leq])^2$ is normal or just pseudo-normal. For example, if $X$ is a $\lambda$ set, then $(X[\leq])^2$ is pseudo-normal but assuming CH there is an $X$ concentrated on a countable dense subset (so not a $\lambda$-set) but still $(X[\leq])^2$ is normal.

==> newheader.tex <==
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{cancel}
\usepackage{amsmath}
\usepackage{mdframed}
\usepackage{hyperref}

\usepackage{array,booktabs}
\usepackage{bm}
\usepackage{tcolorbox}
\usepackage{enumitem}
\usepackage{amssymb}
\usepackage{enumitem}
\usepackage{tikz}
% Please do not remove any existing theorem
\DeclareMathOperator{\rad}{rad}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\closure}{cl}
\DeclareMathOperator{\dir}{dir}
\DeclareMathOperator{\cf}{cf}
\DeclareMathOperator{\add}{add}
\DeclareMathOperator{\ci}{ci}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\non}{non}
\DeclareMathOperator{\nul}{null}

\providecommand*{\claimautorefname}{Claim}

\newtheoremstyle{less}      % Name of the style
  {1pt}                           % Space above
  {1pt}                           % Space below
  {\itshape}                     % Body font (italic)
  {1em}                              % Indent amount
  {\normalfont}                   % Theorem head font (not bold)
  {.}                             % Punctuation after theorem head
  { }                             % Space after theorem head
  {}     



\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{exercise}{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
%\theoremstyle{less}
\newtheorem{observation}{Observation}
\newtheorem{claim}{Claim}
\newtheorem{plain}[theorem]{}



\newcommand{\centered}[1]{\begin{tabular}{l} #1 \end{tabular}}

\newcommand{\partdf}[3][]{\frac{\partial^{#1} #2}{\partial {#3}^{#1}}}
\newcommand{\df}[2]{\frac{d #1}{d #2}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\renewcommand{\S}{\mathbb{S}}
\newcommand{\Ss}{\mathcal{S}}
\newcommand{\Aa}{\mathcal{A}}
\newcommand{\Bb}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dd}{\mathcal{D}}
\newcommand{\Ee}{\mathcal{E}}
\newcommand{\Ff}{\mathcal{F}}
\newcommand{\Gg}{\mathcal{G}}
\newcommand{\Ii}{\mathcal{I}}
\newcommand{\Kk}{\mathcal{K}}
\newcommand{\Ll}{\mathcal{L}}
\newcommand{\Mm}{\mathcal{M}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\Pp}{\mathcal{P}}
\newcommand{\Vv}{\mathcal{V}}
\newcommand{\Uu}{\mathcal{U}}


\newcommand{\Real}{\text{Re }}
\newcommand{\Imagine}{\text{Im }}
\newcommand{\Hol}{\mathcal{H}}
\newcommand{\dif}{\text{ d}}
\newcommand{\WLOG}{\textit{wlog.}}
\newcommand{\bb}{\mathfrak{b}}
\newcommand{\dd}{\mathfrak{d}}
\newcommand{\UU}{\mathfrak{U}}
\newcommand{\ccc}{\textit{ccc.}}


\newcounter{alphsubsection}[section]
\renewcommand{\thealphsubsection}{\alph{alphsubsection}}
\newcommand{\alphsubsection}[1]{%
  \refstepcounter{alphsubsection}%
  \paragraph{\thealphsubsection.\ #1}%
}


% Create a separate counter for alphabetic subsections
\newcounter{Alphsubsection}[section] % Reset at each new section
\renewcommand{\theAlphsubsection}{\thesection.\Alph{Alphsubsection}}

% Define \AlphSubsection command
\newcommand{\AlphSubsection}[1]{%
  \refstepcounter{Alphsubsection}%
  \subsection*{\theAlphsubsection\ #1}%
  \addcontentsline{toc}{subsection}{\theAlphsubsection\ #1}%
}


\newtcolorbox{mybox}[3][]
{
  colframe = #2!25,
  colback  = #2!10,
  coltitle = #2!20!black,  
  title    = {#3},
  #1,
}

\newtcolorbox{simplebox}{
  colframe=black,    % black frame
  colback=white,     % white background
  boxrule=0.5pt,     % thin border
  arc=0mm,           % rounded corners
  left=1mm,          % padding left
  right=1mm,         % padding right
  top=1mm,           % padding top
  bottom=1mm         % padding bottom
}
